GUBS Upper Bound Solver (Extended Abstract)

In this extended abstract we present the GUBS Upper Bound Solver. GUBS is a dedicated constraint solver over the naturals for inequalities formed over uninterpreted function symbols and standard arithmetic operations. GUBS now forms the backbone of HoSA, a tool for analysing space and time complexity of higher-order functional programs automatically. We give insights about the implemen- tation and report different case studies.

==> eptcsdata.tex <==
\providecommand{\firstpage}{17}
\providecommand{\publicationstatus}{G. Bonfante, G. Moser (Eds.): 8th Workshop on Developments in\\ Implicit Computational complExity and 5th Workshop on Foundational\\ and Practical Aspects of Resource Analysis
(DICE-FOPARA 2017)\\
EPTCS 248, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.248.6}{10.4204/EPTCS.248.6}}
\pdfoutput=1

